Optimizing Logical Execution Time Model for Both Determinism and Low Latency

The Logical Execution Time (LET) programming model has recently received considerable attention, particularly because of its timing and dataflow determinism. In LET, task computation appears always to take the same amount of time (called the task's LET interval), and the task reads (resp. writes) at the beginning (resp. end) of the interval. Compared to other communication mechanisms, such as implicit communication and Dynamic Buffer Protocol (DBP), LET performs worse on many metrics, such as end-to-end latency (including reaction time and data age) and time disparity jitter. Compared with the default LET setting, the flexible LET (fLET) model shrinks the LET interval while still guaranteeing schedulability by introducing the virtual offset to defer the read operation and using the virtual deadline to move up the write operation. Therefore, fLET has the potential to significantly improve the end-to-end timing performance while keeping the benefits of deterministic behavior on timing and dataflow. To fully realize the potential of fLET, we consider the problem of optimizing the assignments of its virtual offsets and deadlines. We propose new abstractions to describe the task communication pattern and new optimization algorithms to explore the solution space efficiently. The algorithms leverage the linearizability of communication patterns and utilize symbolic operations to achieve efficient optimization while providing a theoretical guarantee. The framework supports optimizing multiple performance metrics and guarantees bounded suboptimality when optimizing end-to-end latency. Experimental results show that our optimization algorithms improve upon the default LET and its existing extensions and significantly outperform implicit communication and DBP in terms of various metrics, such as end-to-end latency, time disparity, and its jitter.

==> notes_to_schepherd.tex <==
Dear Shepherd,

Thank you very much for being willing to assist in enhancing this paper. We have updated the paper draft to address the mentioned questions. Specifically:
- The "theorem 7" in the submitted version is now numbered as theorem 6, and its detailed proof is provided on page 8. (Following reviewer D, we reformulated "theorem 3" in the submitted version into an observation, resulting in changes to the theorem indexes)
- The pseudo-code of algorithm 1 has been re-written, and a detailed explanation has been added in the paragraph above the pseudo-code on page 9.
- Various presentation issues have been rectified. These changes can be easily seen from the "difference.pdf" in the attachment. 
- Following review B, we also added a realistic case study experiment on page 12.

Please let us know if there are any further modification suggestions. Your feedback is greatly appreciated. Thanks!

Best regards,
The Authors

==> notes_to_shepherd2.tex <==
Dear Shepherd,

Thank you again for carefully reviewing the paper and mentioning these important questions. We have updated the paper accordingly and updated the draft paper to "draft2.pdf". As before, we also provided a "diff2.pdf" file to highlight the modification differences. However, due to LATEX issues, we just noticed that we cannot highlight the modification changes in the pseudo-code, so we just put the modified pseudo-code in "diff2.pdf" without highlighting it. 

- Algorithm 1, "ELP_Set.RemoveWorseELP(ELP Set, worsePatterns)": we removed the function argument "ELP\_Set" to avoid confusion. The purpose of this function is to remove unvisited ELP from $ELP\_Set$ based on the comparison with worsePatterns; it does not necessarily need "ELP" (see changes in ["draft2.pdf", page 9, right column, Algorithm 1, line 20]);

- In the text discussing Algorithm 1, we replaced "ELP\_{unv}" with "the unvisited ELP" to avoid confusion (see changes in ["draft2.pdf", page 9, left column] and ["diff2.pdf", page 9, right column]);

- The worsePatterns FIFO queue will "pop" elements immediately after its size exceeds the limit. For better clarification, we added this condition this time (see changes in ["draft2.pdf", page 9, right column, Algorithm 1, lines 13-14]).

- About the data structure "worsePatterns": we added more explanation in the paper: It is a FIFO queue because more recent communication patterns are more likely to trigger the skip conditions in Corollary 1 during communication pattern enumeration. The capacity size is experimentally set to 50: a larger capacity incurs more computation overhead when a communication pattern cannot be skipped, while a smaller size implies fewer skipped patterns (see changes in ["draft2.pdf", page 9, left column, bottom] and ["diff2.pdf", page 9, right column, top]).

- Reviewer D, comment 8: the ELP is infeasible because no solutions can satisfy the linear inequalities associated with the ELP (see changes in ["draft2.pdf", page 5, right column, Example 4] and ["diff2.pdf", page 5, right column, Example 4]).

- The two last points have been addressed accordingly.

Please let us know if there are any further suggestions for modification. Your feedback is greatly appreciated. Thanks!

Best regards, 

The Authors

==> notes_to_shepherd3.tex <==
Dear Shepherd,

Thank you so much for recognizing the paper and providing these further suggestions, especially the last comment. We have modified the paper accordingly, and you can find the changes on page 9 in "diff3.pdf" and "draft3.pdf". More specifically,

- About the more recent communication patterns: they have more edge communication patterns that are the same as the next communication patterns to evaluate, therefore are more likely to satisfy corollary 1;

- We will try to add this experiment about the queue size in the future version

- About the function "RemoveWorseELP": the major purpose is skipping partial GLPs rather than complete GLPs to achieve a significant speed-up. This is because skipping a partial GLP also implicitly skips all the partial and complete GLPs that contain the skipped partial GLP, and therefore brings big speed improvements.

Apart from these things, we also want to sincerely thank you for your patience and all the time that you devoted to this paper. The contact author is not a sophisticated writer and he also often struggles with paper editing and meeting the page limit. But we're sure that he will learn his lessons and make future submissions more clear and better.

Thanks!

Best Regards,
Authors
